ScaleNAS: One-Shot Learning of Scale-Aware Representations for Visual Recognition

Scale variance among different sizes of body parts and objects is a challenging problem for visual recognition tasks. Existing works usually design dedicated backbone or apply Neural architecture Search(NAS) for each task to tackle this challenge. However, existing works impose significant limitations on the design or search space. To solve these problems, we present ScaleNAS, a one-shot learning method for exploring scale-aware representations. ScaleNAS solves multiple tasks at a time by searching multi-scale feature aggregation. ScaleNAS adopts a flexible search space that allows an arbitrary number of blocks and cross-scale feature fusions. To cope with the high search cost incurred by the flexible space, ScaleNAS employs one-shot learning for multi-scale supernet driven by grouped sampling and evolutionary search. Without further retraining, ScaleNet can be directly deployed for different visual recognition tasks with superior performance. We use ScaleNAS to create high-resolution models for two different tasks, ScaleNet-P for human pose estimation and ScaleNet-S for semantic segmentation. ScaleNet-P and ScaleNet-S outperform existing manually crafted and NAS-based methods in both tasks. When applying ScaleNet-P to bottom-up human pose estimation, it surpasses the state-of-the-art HigherHRNet. In particular, ScaleNet-P4 achieves 71.6% AP on COCO test-dev, achieving new state-of-the-art result.

==> unused/3_old_method.tex <==
% We also use the knowledge distillation technique by using the biggest model as teacher model~\cite{hinton2015distilling, cai2020once, yu2020bignas}.
% During the training of \supernet, each sub-network is not only optimized by true label's cross entropy loss but also the soft label loss from teacher model. 
% The procedure of training \netname are as follows:
% \begin{itemize}
%     \item Obtain teacher model: We activate all the block operation and fusion in the whole search space. train on ImageNet as teacher model.
%     \item Train \netname using teacher model as knowledge distillation 

% \end{itemize}
% As we observe that multi-scale feature fusion boost up performance and break through the performance bottleneck of HRNet. We activate all the fusion connections and block operations as our teacher model. During the searching each subnet not only optimizaed by True label's cross entropy but also the soft label loss from teacher model.

